Dynamic Pricing of Power in Smart-Grid Networks

In this paper we introduce the problem of dynamic pricing of power for smart-grid networks. This is studied within a network utility maximization (NUM) framework in a deterministic setting with a single provider, multiple users and a finite horizon. The provider produces power or buys power in a (deterministic) spot market, and determines a dynamic price to charge the users. The users then adjust their demand in response to the time-varying prices. This is typically categorized as the demand response problem, and we study a progression of related models by focusing on two aspects: 1) the characterization of the structure of the optimal dynamic prices in the Smart Grid and the optimal demand and supply under various interaction with a spot market; 2) a greedy approach to facilitate the solution process of the aggregate NUM problem and the optimality gap between the greedy solution and the optimal one.

==> intro.tex <==
%----------------------------------------------------------
\section{Introduction}

As the Smart Grid takes shape, new possibilities of efficient management of the electric power grid open up. One of these is pricing of electricity to consumers. Currently, temporal variations in the cost of electricity are hidden behind inflexible rate designs. This leads to  inefficiencies with over-consumption during peak times, and under-consumption during off-peak times. It also makes the problem of matching demand and supply, both of which are uncertain, and affect grid stability, particularly acute. In the United States, only 60-100 hours of the year can account for 10-18 percent of the system peak load \cite{FaHlTs10}. Meeting this critical peak load requires installation, operation and maintenance of expensive combustion gas-turbine generators, since these start almost instantaneously.

Dynamic pricing of electricity to consumers can remedy this problem by inducing consumers to switch off or defer some of the non-urgent, non-critical loads. For example, dish-washers in most households have a delayed start option. And yet, only a small fraction of consumers utilize {this feature and} use the appliance later at night at off-peak times. Dynamic pricing can make consumers sensitive to their time and amount of electricity consumption, thus potentially smoothing out peak-time system loads, and enhancing economic efficiency.

Dynamic pricing rate designs are receiving increased attention by state commissions, with the California Public Utilities Commission (CPUC) having set a deadline of 2011 for the state electric utilities to propose dynamic pricing rate structures. These are defined as an electric rate structure that reflects the actual wholesale market conditions. Dynamic pricing can take various forms such as \textit{critical peak-pricing}, \textit{time-of-use pricing} and \textit{real-time pricing}. CPUC defines the real-time price as the rate linked to the actual price in the wholesale hourly electricity market \cite{CPUC08}. Such prices can be communicated to the consumers over the \textit{advanced metering infrastructure} (AMI), or a \textit{smart-grid network} \cite{DoE08} and displayed on a \textit{smart meter}.

\noindent \textit{Literature Overview.} Problems related to {the} design and operation of a Smart Grid are receiving increasing attention. The problem of dynamic pricing to shape demand is typically called \textit{demand response}. There exists a large literature on demand response; the most relevant is \cite{LiChLo10}. This paper formulates the problem of optimal demand response in discrete time over a finite time horizon when users have some storage available, and the formulation can be categorized as a network utility maximization (NUM) problem \rev{(see \cite{Palomar06}, \cite{Chiang07} and the references therein)}.
%\com{Let's provide a few references on NUM, and maybe a few sentences' summary of this class of problems?}
Using Lagrangian duality, it establishes the existence of a solution, and gives a distributed algorithm {based on gradient projection} to compute this solution. {The modeling of various appliances into the proposed optimization framework is also studied.} In \cite{ChLiLoDo11}, a different approach is taken wherein demand is required to match supply, and users bid for load-shedding in an iterative supply function bidding mechanism, that was first proposed in \cite{KlMe89}. Both competitive and Nash equilibrium analysis is provided but the focus is on a single instant, and without storage. In \cite{LaLo11}, the focus is on optimal power flow through the network, wherein existence of a zero duality gap solution is proved. In contrast to aforementioned work, {particularly \cite{LiChLo10}, in this paper we study a progression of related models by focusing on two aspects: 1) the characterization of the structure of the optimal dynamic prices in the Smart Grid and the optimal demand and supply under various interaction with a spot market; 2) a greedy approach to facilitate the solution process of the aggregate NUM and the optimality gap between the greedy solution and the optimal one.}
%\com{We used to have more on related work, which were commented below in the source file. Are we going to add them to this version?}

\rev{Other works have focused on electricity markets. While \cite{RoDaMi10} provides a stability analysis of the wholesale electricity market, \cite{BiRaKhPoVa11} has focused on means for wind power generators to participate in the day-ahead electricity market. The difficulty in this is that wind-power generators cannot enter into binding contracts for a day-ahead power supply without assuming a huge risk. Thus, alternative market architectures are considered in \cite{TaJa11}, wherein entities called ``aggregators" buy power from the wind power generators and participate in the day-ahead markets. The paper proposes optimal mechanisms that the aggregators can use to get the wind power generators to reveal their true distributions, and thus minimize the risk due to uncertainty in supply from the contracted wind power generators. A related paper is \cite{VaWuBi11}, wherein mechanisms for riskless dispatch by the generators are given for use with the current market architecture.}

\noindent \textit{Results and organization of this paper.} {The system model is first presented in Section~\ref{sec:model}, and three related problems are introduced. The first problem {\tt SYSTEM} is a simplified special case of the main model with internalized production cost, which provides a preliminary framework for more realistic refinement. {Its} optimal solution is characterized in Section~\ref{sec:gradient} based on a dual decomposition; moreover, a distributed algorithm to solve {\tt SYSTEM}, which can be readily adapted for problems in the same family, is also proposed. In Section~\ref{sec:spot} we extend the {\tt SYSTEM} problem to the scenario where the provider may purchase in part from a spot market with an exogenous cost to narrow the demand-supply gap. {This is referred to as the %, which summarizes our study of the second problem
{\tt SYS\_SPOT} problem,} and the interaction between the decision of purchase and the spot market price is investigated. We then consider the explicit effect of the production cost {in a} %by proceeding to the
third problem in Section~\ref{sec:optctrl}, and the structure of its optimal control in the single-user scenario is studied. A greedy algorithm to approximate the solution to {\tt SYSTEM} is presented in Section~\ref{sec:greedy}, where an upper bound on the optimality gap is established and heuristics on evaluating this gap are discussed. Numerical results of sample problems are illustrated in Section~\ref{sec:num}. We present an attempt of adopting distributed Newton's method to problems in this work in Section~\ref{sec:newton}, and Section \ref{sec:conclusion} concludes the paper.



